Incremental Learning of Retrievable Skills For Efficient Continual Task Adaptation

Continual Imitation Learning (CiL) involves extracting and accumulating task knowledge from demonstrations across multiple stages and tasks to achieve a multi-task policy. With recent advancements in foundation models, there has been a growing interest in adapter-based CiL approaches, where adapters are established parameter-efficiently for tasks newly demonstrated. While these approaches isolate parameters for specific tasks and tend to mitigate catastrophic forgetting, they limit knowledge sharing among different demonstrations. We introduce IsCiL, an adapter-based CiL framework that addresses this limitation of knowledge sharing by incrementally learning shareable skills from different demonstrations, thus enabling sample-efficient task adaptation using the skills particularly in non-stationary CiL environments. In IsCiL, demonstrations are mapped into the state embedding space, where proper skills can be retrieved upon input states through prototype-based memory. These retrievable skills are incrementally learned on their corresponding adapters. Our CiL experiments with complex tasks in Franka-Kitchen and Meta-World demonstrate robust performance of IsCiL in both task adaptation and sample-efficiency. We also show a simple extension of IsCiL for task unlearning scenarios.

==> table/extension_fig.tex <==
\begin{minipage}{.49\linewidth}
    \includegraphics[width=.95\linewidth]{fig/result_rehearsal.png}
    \caption{
    Evaluation against rehearsal-based methods and \ours with rehearsal. Light colors indicate the difference between FWT and AUC, while dark colors show the final AUC performance.}
    \label{fig:exp_rehearsal}
\end{minipage}
\hfill
\begin{minipage}{.49\linewidth}
    \includegraphics[width=.95\linewidth]{fig/fig_constraint.png}
    \caption{
    Comparison is made in a scenario with limited computing resources. 
     Light colors indicate the difference between FWT and AUC, while dark colors show the final AUC performance.}
    \label{fig:exp_computation}
\end{minipage}



==> table/learning_2.tex <==

\begin{table*}[t]
    \centering
    \caption{Evolving Kitchen Results }   
    \vskip 0.1 in
    \begin{adjustbox}{width=1.0 \textwidth}
    \begin{tabular}{l|ccccccccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Stream}(Total phase) }
    & \multicolumn{3}{c}{Environment IL-Train}
    & \multicolumn{3}{c}{Environment IL-Seen}
    & \multicolumn{3}{c}{Environment IL-UnSeen}
    \\
    
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    
    
    CL-algorithm
    & \metricc
    & \metricb
    & \metrica
    & \metricc
    & \metricb
    & \metrica
    & \metricc
    & \metricb
    & \metrica\\

    
    \midrule
    Seq-FT
    & 75.0{\color{gray}\scriptsize$\pm$1.8}
    & -58.0{\color{gray}\scriptsize$\pm$2.3}
    & 24.3{\color{gray}\scriptsize$\pm$0.3}
    & 77.5{\color{gray}\scriptsize$\pm$2.3}
    & -67.3{\color{gray}\scriptsize$\pm$2.5}
    & 18.8{\color{gray}\scriptsize$\pm$0.5}
    & 70.3{\color{gray}\scriptsize$\pm$6.5}
    & -63.5{\color{gray}\scriptsize$\pm$7.2}
    & 14.0{\color{gray}\scriptsize$\pm$1.5}
    \\

    EWC
    & 48.8{\color{gray}\scriptsize$\pm$2.5}
    & -36.3{\color{gray}\scriptsize$\pm$2.5}
    & 17.3{\color{gray}\scriptsize$\pm$0.0}
    & 55.3{\color{gray}\scriptsize$\pm$3.5}
    & -46.8{\color{gray}\scriptsize$\pm$1.3}
    & 14.0{\color{gray}\scriptsize$\pm$1.8}
    & 44.5{\color{gray}\scriptsize$\pm$2.0}
    & -40.3{\color{gray}\scriptsize$\pm$3.0}
    & 9.0{\color{gray}\scriptsize$\pm$0.8}
    \\

    \midrule
    
    One Adapter
    & 88.8{\color{gray}\scriptsize$\pm$2.5}
    & -67.5{\color{gray}\scriptsize$\pm$3.0}
    & 29.0{\color{gray}\scriptsize$\pm$0.5}
    & 89.5{\color{gray}\scriptsize$\pm$2.3}
    & -78.0{\color{gray}\scriptsize$\pm$2.0}
    & 20.8{\color{gray}\scriptsize$\pm$0.5}
    & \textbf{76.5{\color{gray}\scriptsize$\pm$3.3}}
    & -70.8{\color{gray}\scriptsize$\pm$3.8}
    & 14.2{\color{gray}\scriptsize$\pm$0.8}
    \\
    
    LAE
    & 84.5{\color{gray}\scriptsize$\pm$3.0}
    & -59.3{\color{gray}\scriptsize$\pm$3.0}
    & 31.8{\color{gray}\scriptsize$\pm$0.8}
    & 81.3{\color{gray}\scriptsize$\pm$6.8}
    & -63.0{\color{gray}\scriptsize$\pm$6.3}
    & 26.0{\color{gray}\scriptsize$\pm$1.5}
    & 16.0{\color{gray}\scriptsize$\pm$1.5}
    & -14.8{\color{gray}\scriptsize$\pm$1.5}
    & 3.0{\color{gray}\scriptsize$\pm$0.3}
    \\
    \midrule
    
    L2M % Basic 
    & 40.8{\color{gray}\scriptsize$\pm$1.0}
    & -12.8{\color{gray}\scriptsize$\pm$2.5}
    & 28.7{\color{gray}\scriptsize$\pm$1.5}
    & 34.3{\color{gray}\scriptsize$\pm$1.5} %
    & -19.3{\color{gray}\scriptsize$\pm$4.0}
    & 16.3{\color{gray}\scriptsize$\pm$4.8}
    & 26.0{\color{gray}\scriptsize$\pm$1.0} %
    & -13.8{\color{gray}\scriptsize$\pm$2.3}
    & 13.5{\color{gray}\scriptsize$\pm$1.3}
    \\

    DACo+L2M
    & 56.5{\color{gray}\scriptsize$\pm$1.0}
    & -3.8{\color{gray}\scriptsize$\pm$1.8}
    & 53.0{\color{gray}\scriptsize$\pm$2.0}
    & 50.2{\color{gray}\scriptsize$\pm$2.0}
    & -2.0{\color{gray}\scriptsize$\pm$2.5}
    & 49.0{\color{gray}\scriptsize$\pm$0.8}
    & 29.8{\color{gray}\scriptsize$\pm$1.3}
    & 0.3{\color{gray}\scriptsize$\pm$1.0}
    & 30.0{\color{gray}\scriptsize$\pm$1.0}
    \\
    

    \ours(ours)
    & \textbf{88.5{\color{gray}\scriptsize$\pm$3.0}}
    & \textbf{-3.0{\color{gray}\scriptsize$\pm$3.0}}
    & \textbf{85.5{\color{gray}\scriptsize$\pm$0.3}}
    & \textbf{89.8{\color{gray}\scriptsize$\pm$2.5}}
    & \textbf{-4.8{\color{gray}\scriptsize$\pm$15.0}}
    & \textbf{84.5{\color{gray}\scriptsize$\pm$2.0}}
    & 73.5{\color{gray}\scriptsize$\pm$1.3}
    & \textbf{1.3{\color{gray}\scriptsize$\pm$2.8}}
    & \textbf{74.3{\color{gray}\scriptsize$\pm$1.8}}
    \\
    
    \midrule
    
    Oracle ID 
    & 87.3{\color{gray}\scriptsize$\pm$4.8}
    & -
    & -
    & 88.0{\color{gray}\scriptsize$\pm$2.3}
    & -
    & -
    & 85.0{\color{gray}\scriptsize$\pm$2.0}
    & -
    & -
    \\
    
    Multi-task
    & -
    & -
    & 92.3{\color{gray}\scriptsize$\pm$0.5}
    & -
    & -
    & 93.8{\color{gray}\scriptsize$\pm$2.0}
    & -
    & -
    & 80.8{\color{gray}\scriptsize$\pm$3.5}
    \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{table:mainEK}
\end{table*}





% \begin{table*}[t]
%     \centering
%     \caption{Evolving Kitchen results: domain varying configuration analysis }   
%     \vskip 0.1 in
%     \begin{adjustbox}{width=1.0 \textwidth}
%     \begin{tabular}{l|c|ccccccccc|c}
%     \toprule
%     \multicolumn{2}{l}{\textbf{Stream}(Total phase) }
%     & \multicolumn{3}{c}{Evolving Kitchen-Single(24)}
%     & \multicolumn{3}{c}{Evolving Kitchen-Mild(24)}
%     & \multicolumn{3}{c}{Evolving Kitchen-Large(24)}
%     & \multicolumn{1}{c}{Avg.}\\
    
%     \cmidrule(lr){1-2}
%     \cmidrule(lr){3-5}
%     \cmidrule(lr){6-8}
%     \cmidrule(lr){9-11}
%     \cmidrule(lr){12-12}\
    
%     CL-algorithm
%     & Type
%     & \metricc
%     & \metricb
%     & \metrica
%     & \metricc
%     & \metricb
%     & \metrica
%     & \metricc
%     & \metricb
%     & \metrica
%     & \metrica\\
%     \midrule
%     Seq-FT
%     & \multirow{3}{*}{Full}
%     & 75.0{\color{gray}\scriptsize$\pm$1.8}
%     & -58.0{\color{gray}\scriptsize$\pm$2.3}
%     & 24.3{\color{gray}\scriptsize$\pm$0.3}
%     & 77.5{\color{gray}\scriptsize$\pm$2.3}
%     & -67.3{\color{gray}\scriptsize$\pm$2.5}
%     & 18.8{\color{gray}\scriptsize$\pm$0.5}
%     & 70.3{\color{gray}\scriptsize$\pm$6.5}
%     & -63.5{\color{gray}\scriptsize$\pm$7.2}
%     & 14.0{\color{gray}\scriptsize$\pm$1.5}
%     & 19.0\\

%     EWC
%     &
%     & 48.8{\color{gray}\scriptsize$\pm$2.5}
%     & -36.3{\color{gray}\scriptsize$\pm$2.5}
%     & 17.3{\color{gray}\scriptsize$\pm$0.0}
%     & 55.3{\color{gray}\scriptsize$\pm$3.5}
%     & -46.8{\color{gray}\scriptsize$\pm$1.3}
%     & 14.0{\color{gray}\scriptsize$\pm$1.8}
%     & 44.5{\color{gray}\scriptsize$\pm$2.0}
%     & -40.3{\color{gray}\scriptsize$\pm$3.0}
%     & 9.0{\color{gray}\scriptsize$\pm$0.8}
%     & 13.4\\

%     EWC(L2)
%     &
%     & 17.3{\color{gray}\scriptsize$\pm$1.0}
%     & -10.3{\color{gray}\scriptsize$\pm$1.0}
%     & 8.3{\color{gray}\scriptsize$\pm$0.8}
%     & 17.3{\color{gray}\scriptsize$\pm$1.0}
%     & -10.3{\color{gray}\scriptsize$\pm$1.0}
%     & 8.3{\color{gray}\scriptsize$\pm$0.8}
%     & 11.5{\color{gray}\scriptsize$\pm$0.3}
%     & -9.5{\color{gray}\scriptsize$\pm$0.5}
%     & 3.0{\color{gray}\scriptsize$\pm$0.5}
%     & 6.5\\
%     \midrule
    
%     One Adapter
%     & \multirow{2}{*}{Accum.}
%     & 88.8{\color{gray}\scriptsize$\pm$2.5}
%     & -67.5{\color{gray}\scriptsize$\pm$3.0}
%     & 29.0{\color{gray}\scriptsize$\pm$0.5}
%     & 89.5{\color{gray}\scriptsize$\pm$2.3}
%     & -78.0{\color{gray}\scriptsize$\pm$2.0}
%     & 20.8{\color{gray}\scriptsize$\pm$0.5}
%     & \textbf{76.5{\color{gray}\scriptsize$\pm$3.3}}
%     & -70.8{\color{gray}\scriptsize$\pm$3.8}
%     & 14.2{\color{gray}\scriptsize$\pm$0.8}
%     & 21.3\\
    
%     LAE
%     & 
%     & 84.5{\color{gray}\scriptsize$\pm$3.0}
%     & -59.3{\color{gray}\scriptsize$\pm$3.0}
%     & 31.8{\color{gray}\scriptsize$\pm$0.8}
%     & 81.3{\color{gray}\scriptsize$\pm$6.8}
%     & -63.0{\color{gray}\scriptsize$\pm$6.3}
%     & 26.0{\color{gray}\scriptsize$\pm$1.5}
%     & 16.0{\color{gray}\scriptsize$\pm$1.5}
%     & -14.8{\color{gray}\scriptsize$\pm$1.5}
%     & 3.0{\color{gray}\scriptsize$\pm$0.3}
%     & 20.3\\
%     \midrule
    
%     L2M % Basic 
%     & \multirow{3}{*}{Matching}
%     & 40.8{\color{gray}\scriptsize$\pm$1.0}
%     & -12.8{\color{gray}\scriptsize$\pm$2.5}
%     & 28.7{\color{gray}\scriptsize$\pm$1.5}
%     & 34.3{\color{gray}\scriptsize$\pm$1.5} %
%     & -19.3{\color{gray}\scriptsize$\pm$4.0}
%     & 16.3{\color{gray}\scriptsize$\pm$4.8}
%     & 26.0{\color{gray}\scriptsize$\pm$1.0} %
%     & -13.8{\color{gray}\scriptsize$\pm$2.3}
%     & 13.5{\color{gray}\scriptsize$\pm$1.3}
%     & 19.5\\

%     DACo+L2M
%     & 
%     & 56.5{\color{gray}\scriptsize$\pm$1.0}
%     & -3.8{\color{gray}\scriptsize$\pm$1.8}
%     & 53.0{\color{gray}\scriptsize$\pm$2.0}
%     & 50.2{\color{gray}\scriptsize$\pm$2.0}
%     & -2.0{\color{gray}\scriptsize$\pm$2.5}
%     & 49.0{\color{gray}\scriptsize$\pm$0.8}
%     & 29.8{\color{gray}\scriptsize$\pm$1.3}
%     & 0.3{\color{gray}\scriptsize$\pm$1.0}
%     & 30.0{\color{gray}\scriptsize$\pm$1.0}
%     & 44.0\\
    

%     \ours(ours)
%     &
%     & \textbf{88.5{\color{gray}\scriptsize$\pm$3.0}}
%     & \textbf{-3.0{\color{gray}\scriptsize$\pm$3.0}}
%     & \textbf{85.5{\color{gray}\scriptsize$\pm$0.3}}
%     & \textbf{89.8{\color{gray}\scriptsize$\pm$2.5}}
%     & \textbf{-4.8{\color{gray}\scriptsize$\pm$15.0}}
%     & \textbf{84.5{\color{gray}\scriptsize$\pm$2.0}}
%     & 73.5{\color{gray}\scriptsize$\pm$1.3}
%     & \textbf{1.3{\color{gray}\scriptsize$\pm$2.8}}
%     & \textbf{74.3{\color{gray}\scriptsize$\pm$1.8}}
%     & \textbf{81.4}\\
    
%     \midrule
    
%     Oracle ID 
%     &  \multirow{2}{*}{Oracle}
%     & 87.3{\color{gray}\scriptsize$\pm$4.8}
%     & -
%     & -
%     & 88.0{\color{gray}\scriptsize$\pm$2.3}
%     & -
%     & -
%     & 85.0{\color{gray}\scriptsize$\pm$2.0}
%     & -
%     & -
%     & -\\
    
%     Multi-task
%     & 
%     & -
%     & -
%     & 92.3{\color{gray}\scriptsize$\pm$0.5}
%     & -
%     & -
%     & 93.8{\color{gray}\scriptsize$\pm$2.0}
%     & -
%     & -
%     & 80.8{\color{gray}\scriptsize$\pm$3.5}
%     & -\\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{table:mainEK}
% \end{table*}



==> table/learning_adapt_leg.tex <==
\begin{table*}[t]
    \centering
    \caption{
    % \textcolor{red}{to be deprecated -> changed to the graph}
    Task adaptation efficiency Evolving world results for varying unseen condition of environment. \textit{Combineable} refers to tasks that can be solved by combining learned trajectories. \textit{In-distribution} refers to environments that can be handled by models trained on given training data in a multi-task learning setup. \textit{Unseen} refers to a completely new evaluation set where the combination of objects and the sequence of sub-tasks are given in the environment. Model is trained in Evolving World-complete. for unseen task evaluation, only the task instruction and sub-goal is given at initial phase.
    }   
    \vskip 0.1 in
    \begin{adjustbox}{width=1.0 \textwidth}
    \begin{tabular}{l|ccccccccc}
    \toprule
    \multicolumn{1}{l}{\textbf{Stream} }
    & \multicolumn{3}{c}{Evolving World Combinable}
    & \multicolumn{3}{c}{Evolving World In-distribution}
    & \multicolumn{3}{c}{Evolving World Unseen}
    \\
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    CL-algorithm
    & \metricc
    & \metricb
    & \metrica
    & \metricc
    & \metricb
    & \metrica
    & \metricc
    & \metricb
    & \metrica\\
    \midrule
    Pre-trained
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    \midrule
    Seq-FT
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    SPiRL-FT
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    EWC
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    Seq-LoRA
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    % EWC-LoRA
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % %
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % %
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % & 0.0{\color{gray}\scriptsize$\pm$0.0}
    % \\
    \midrule
    L2M
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    L2M+TE
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    \ours (ours)
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    \midrule
    Multi-task
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    %
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    & 0.0{\color{gray}\scriptsize$\pm$0.0}
    \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{table:main_unseen_leg}
    \vskip -0.1 in
    
\end{table*}




==> table/multiple_example.tex <==
\begin{minipage}{.49\linewidth}
    \includegraphics[width=.95\linewidth]{fig/result_rehearsal.png}
    \caption{
    Rehearsal comparison
    % Evaluation against rehearsal-based methods and \ours with rehearsal. Light colors indicate the difference between FWT and AUC, while dark colors show the final AUC performance.
    }
    \label{fig:exp_rehearsal}
    % \caption{Limited training resource}   
    % \vskip 0.1 in
    % \begin{adjustbox}{width=0.99 \columnwidth }
    % \begin{tabular}{l|c|ccc}
    % \toprule
    
    % \multicolumn{2}{l}{\textbf{Stream}(Total phase)}
    % & \multicolumn{3}{c}{Evolving kitchen-Single(24)}\\
    
    % \cmidrule(lr){1-2}
    % \cmidrule(lr){3-5}
    
    % Epoch/phase & Baselines
    % & \metricc
    % & \metricb
    % & \metrica \\
    % \midrule

    % \multirow{3}{*}{100}&L2M
    % & 26.3{\color{gray}\scriptsize$\pm$2.3}
    % & -13.0{\color{gray}\scriptsize$\pm$1.9}
    % & 14.2{\color{gray}\scriptsize$\pm$3.0}\\
    % &L2M+TE
    % & 28.1{\color{gray}\scriptsize$\pm$1.6}
    % & 0.3{\color{gray}\scriptsize$\pm$1.7}
    % & 28.5{\color{gray}\scriptsize$\pm$0.2}\\
    % &\ours
    % & 33.5{\color{gray}\scriptsize$\pm$4.3}
    % & -1.0{\color{gray}\scriptsize$\pm$1.5}
    % & 32.8{\color{gray}\scriptsize$\pm$4.3}\\
    % \midrule
    
    % \multirow{3}{*}{500}&L2M
    % & 25.3{\color{gray}\scriptsize$\pm$7.4}
    % & -10.6{\color{gray}\scriptsize$\pm$3.6}
    % & 15.0{\color{gray}\scriptsize$\pm$4.1}\\

    % &L2M+TE
    % & 30.3{\color{gray}\scriptsize$\pm$0.4}
    % & 0.3{\color{gray}\scriptsize$\pm$0.3}
    % & 30.5{\color{gray}\scriptsize$\pm$0.4}\\
    
    % &\ours
    % & 54.5{\color{gray}\scriptsize$\pm$10.0}
    % & 7.5{\color{gray}\scriptsize$\pm$2.8}
    % & 61.0{\color{gray}\scriptsize$\pm$11.3}\\
    % \midrule

    % \multirow{3}{*}{1000}&L2M
    % & 24.0{\color{gray}\scriptsize$\pm$4.8}
    % & -1.4{\color{gray}\scriptsize$\pm$2.8}
    % & 22.6{\color{gray}\scriptsize$\pm$5.3}\\

    % &L2M+TE
    % & 32.6{\color{gray}\scriptsize$\pm$0.6}
    % & 0.5{\color{gray}\scriptsize$\pm$0.6}
    % & 33.0{\color{gray}\scriptsize$\pm$0.2}\\

    % &\ours
    % & 80.5{\color{gray}\scriptsize$\pm$2.3}
    % & -2.0{\color{gray}\scriptsize$\pm$2.3}
    % & 79.0{\color{gray}\scriptsize$\pm$2.5}\\
    
    % \midrule 
    % \multirow{3}{*}{3000 (Table ~\ref{table:mainEK})}&L2M
    % & 40.8{\color{gray}\scriptsize$\pm$1.8}
    % & -12.8{\color{gray}\scriptsize$\pm$2.5}
    % & 28.7{\color{gray}\scriptsize$\pm$1.5}\\

    % &DACo+L2M
    % & 56.5{\color{gray}\scriptsize$\pm$1.0}
    % & -3.8{\color{gray}\scriptsize$\pm$1.8}
    % & 53.0{\color{gray}\scriptsize$\pm$2.0}\\

    % &\ours
    % & 88.5{\color{gray}\scriptsize$\pm$3.0}
    % & -3.0{\color{gray}\scriptsize$\pm$3.0}
    % & 85.5{\color{gray}\scriptsize$\pm$0.3}\\

    % \bottomrule
    % \end{tabular}
    % \end{adjustbox}
    % \label{table:limitresource}
\end{minipage}
\hfill
\begin{minipage}{.49\linewidth}
    \includegraphics[width=.95\linewidth]{fig/fig_constraint.png}
    \caption{
    Training resource comparison
    % Comparison is made in a scenario with limited computing resources. 
    %  Light colors indicate the difference between FWT and AUC, while dark colors show the final AUC performance.
    }
    \label{fig:exp_epoch}
    % \centering
    % \caption{Rehearsal comparison}   
    % \vskip 0.1 in
    % \begin{adjustbox}{width=0.9 \columnwidth }
    % \begin{tabular}{c|l|ccc}
    % \toprule
    
    % \multicolumn{2}{l}{\textbf{Stream}(Total phase)}
    % & \multicolumn{3}{c}{Evolving Kitchen-Single(24)}\\
    
    % \cmidrule(lr){1-2}
    % \cmidrule(lr){3-5}
    
    % Baselines& rehearsal
    % & \metricc
    % & \metricb
    % & \metrica \\
    % \midrule

    % \multirow{4}{*}{ER}&  50
    % & 85.0{\color{gray}\scriptsize$\pm$3.3}
    % & -37.8{\color{gray}\scriptsize$\pm$2.3}
    % & 51.7{\color{gray}\scriptsize$\pm$1.5}\\
    
    % & 100
    % & 82.8{\color{gray}\scriptsize$\pm$1.5}
    % & -31.3{\color{gray}\scriptsize$\pm$4.5}
    % & 55.0{\color{gray}\scriptsize$\pm$2.8}\\

    % & 500
    % & 82.3{\color{gray}\scriptsize$\pm$2.5}
    % & -15.0{\color{gray}\scriptsize$\pm$3.3}
    % & 66.0{\color{gray}\scriptsize$\pm$0.3}\\
    
    % & 1000
    % & 81.5{\color{gray}\scriptsize$\pm$1.5}
    % & -10.3{\color{gray}\scriptsize$\pm$2.8}
    % & 72.0{\color{gray}\scriptsize$\pm$1.5}\\
    % \midrule

    % \multirow{4}{*}{L2M + ER}&  50
    % & 85.0{\color{gray}\scriptsize$\pm$3.3}
    % & -37.8{\color{gray}\scriptsize$\pm$2.3}
    % & 51.7{\color{gray}\scriptsize$\pm$1.5}\\
    
    % & 100
    % & 82.8{\color{gray}\scriptsize$\pm$1.5}
    % & -31.3{\color{gray}\scriptsize$\pm$4.5}
    % & 55.0{\color{gray}\scriptsize$\pm$2.8}\\

    % & 500
    % & 82.3{\color{gray}\scriptsize$\pm$2.5}
    % & -15.0{\color{gray}\scriptsize$\pm$3.3}
    % & 66.0{\color{gray}\scriptsize$\pm$0.3}\\
    
    % & 1000
    % & 81.5{\color{gray}\scriptsize$\pm$1.5}
    % & -10.3{\color{gray}\scriptsize$\pm$2.8}
    % & 72.0{\color{gray}\scriptsize$\pm$1.5}\\
    % \midrule
    
    % \ours & 0
    % & 88.5{\color{gray}\scriptsize$\pm$3.0}
    % & -3.0{\color{gray}\scriptsize$\pm$3.0}
    % & 85.5{\color{gray}\scriptsize$\pm$0.3}\\

    % \bottomrule
    % \end{tabular}
    % \end{adjustbox}
    % \label{table:rehearsal}
\end{minipage}


%%% ablations 
% \caption{Framework Ablation}   
    % \vskip 0.1 in
    % \begin{adjustbox}{width=0.9 \columnwidth }
    % \begin{tabular}{l|ccc}
    % \toprule
    
    % \multicolumn{1}{c}{\textbf{Stream}(Total phase)}
    % & \multicolumn{3}{c}{Evolving World(20)}\\
    
    % \cmidrule(lr){1-1}
    % \cmidrule(lr){2-4}
    
    % Ablations 
    % & \metricc
    % & \metricb
    % & \metrica \\

    % \midrule
    % \ours w/o meta initialization
    % % without initialization
    % & 65.5{\color{gray}\scriptsize$\pm$0.8}
    % & -2.0{\color{gray}\scriptsize$\pm$1.0}
    % & 63.5{\color{gray}\scriptsize$\pm$0.5}\\
    
    % \ours naive initialization
    % % see every skills are complement dataset
    % & 67.8{\color{gray}\scriptsize$\pm$5.0}
    % & 2.0{\color{gray}\scriptsize$\pm$5.0}
    % & 69.5{\color{gray}\scriptsize$\pm$1.5}\\

    % \ours w/o regularization
    % % see every skills are complement dataset
    % & 67.8{\color{gray}\scriptsize$\pm$5.0}
    % & 2.0{\color{gray}\scriptsize$\pm$5.0}
    % & 69.5{\color{gray}\scriptsize$\pm$1.5}\\
    % \midrule
    
    % \ours naive incremental
    % % see every skills are complement dataset
    % & 67.8{\color{gray}\scriptsize$\pm$5.0}
    % & 2.0{\color{gray}\scriptsize$\pm$5.0}
    % & 69.5{\color{gray}\scriptsize$\pm$1.5}\\

    % \ours only prototype
    % % see every skills are complement dataset
    % & 67.8{\color{gray}\scriptsize$\pm$5.0}
    % & 2.0{\color{gray}\scriptsize$\pm$5.0}
    % & 69.5{\color{gray}\scriptsize$\pm$1.5}\\
    
    % % \ours w/o skill accumulation
    % % % no update for learned dataset
    % % & 13.3{\color{gray}\scriptsize$\pm$0.3}
    % % & -0.5{\color{gray}\scriptsize$\pm$0.3}
    % % & 13.0{\color{gray}\scriptsize$\pm$0.3}\\

    % \midrule
    % \ours 
    % & 76.5{\color{gray}\scriptsize$\pm$1.5}
    % & -1.0{\color{gray}\scriptsize$\pm$1.8}
    % & 75.5{\color{gray}\scriptsize$\pm$1.8}\\
    
    % \bottomrule
    % \end{tabular}
    % \end{adjustbox}
    % \label{table:ablation}
%%% ablations end

    % % Table 3
    % \centering
    % \caption{Limited training resource}   
    % \vskip 0.1 in
    % \begin{adjustbox}{width=0.5 \columnwidth }
    % \begin{tabular}{l|c|ccc}
    % \toprule
    
    % \multicolumn{2}{l}{\textbf{Stream}(Total phase)}
    % & \multicolumn{3}{c}{Evolving kitchen-Single(24)}\\
    
    % \cmidrule(lr){1-2}
    % \cmidrule(lr){3-5}
    
    % Epoch/phase & Baselines
    % & \metricc
    % & \metricb
    % & \metrica \\
    % \midrule

    % \multirow{3}{*}{100}&L2M
    % & 26.3{\color{gray}\scriptsize$\pm$2.3}
    % & -13.0{\color{gray}\scriptsize$\pm$1.9}
    % & 14.2{\color{gray}\scriptsize$\pm$3.0}\\
    % &DACo+L2M
    % & 28.1{\color{gray}\scriptsize$\pm$1.6}
    % & 0.3{\color{gray}\scriptsize$\pm$1.7}
    % & 28.5{\color{gray}\scriptsize$\pm$0.2}\\
    % &\ours
    % & 33.5{\color{gray}\scriptsize$\pm$4.3}
    % & -1.0{\color{gray}\scriptsize$\pm$1.5}
    % & 32.8{\color{gray}\scriptsize$\pm$4.3}\\
    % \midrule
    
    % \multirow{3}{*}{500}&L2M
    % & 25.3{\color{gray}\scriptsize$\pm$7.4}
    % & -10.6{\color{gray}\scriptsize$\pm$3.6}
    % & 15.0{\color{gray}\scriptsize$\pm$4.1}\\

    % &DACo+L2M
    % & 30.3{\color{gray}\scriptsize$\pm$0.4}
    % & 0.3{\color{gray}\scriptsize$\pm$0.3}
    % & 30.5{\color{gray}\scriptsize$\pm$0.4}\\
    
    % &\ours
    % & 54.5{\color{gray}\scriptsize$\pm$10.0}
    % & 7.5{\color{gray}\scriptsize$\pm$2.8}
    % & 61.0{\color{gray}\scriptsize$\pm$11.3}\\
    % \midrule

    % \multirow{3}{*}{1000}&L2M
    % & 24.0{\color{gray}\scriptsize$\pm$4.8}
    % & -1.4{\color{gray}\scriptsize$\pm$2.8}
    % & 22.6{\color{gray}\scriptsize$\pm$5.3}\\

    % &DACo+L2M
    % & 32.6{\color{gray}\scriptsize$\pm$0.6}
    % & 0.5{\color{gray}\scriptsize$\pm$0.6}
    % & 33.0{\color{gray}\scriptsize$\pm$0.2}\\

    % &\ours
    % & 80.5{\color{gray}\scriptsize$\pm$2.3}
    % & -2.0{\color{gray}\scriptsize$\pm$2.3}
    % & 79.0{\color{gray}\scriptsize$\pm$2.5}\\
    
    % \midrule 
    % \multirow{3}{*}{3000 (Table ~\ref{table:mainEK})}&L2M
    % & 40.8{\color{gray}\scriptsize$\pm$1.8}
    % & -12.8{\color{gray}\scriptsize$\pm$2.5}
    % & 28.7{\color{gray}\scriptsize$\pm$1.5}\\

    % &DACo+L2M
    % & 56.5{\color{gray}\scriptsize$\pm$1.0}
    % & -3.8{\color{gray}\scriptsize$\pm$1.8}
    % & 53.0{\color{gray}\scriptsize$\pm$2.0}\\

    % &\ours
    % & 88.5{\color{gray}\scriptsize$\pm$3.0}
    % & -3.0{\color{gray}\scriptsize$\pm$3.0}
    % & 85.5{\color{gray}\scriptsize$\pm$0.3}\\

    % \bottomrule
    % \end{tabular}
    % \end{adjustbox}
    % \label{table:limitresource}
    % \vskip -0.5in
    
